Ensuring accurate stain reproduction in deep generative networks for virtual immunohistochemistry

Immunohistochemistry is a valuable diagnostic tool for cancer pathology. However, it requires specialist labs and equipment, is time-intensive, and is difficult to reproduce. Consequently, a long term aim is to provide a digital method of recreating physical immunohistochemical stains. Generative Adversarial Networks have become exceedingly advanced at mapping one image type to another and have shown promise at inferring immunostains from haematoxylin and eosin. However, they have a substantial weakness when used with pathology images as they can fabricate structures that are not present in the original data. CycleGANs can mitigate invented tissue structures in pathology image mapping but have a related disposition to generate areas of inaccurate staining. In this paper, we describe a modification to the loss function of a CycleGAN to improve its mapping ability for pathology images by enforcing realistic stain replication while retaining tissue structure. Our approach improves upon others by considering structure and staining during model training. We evaluated our network using the Fr\'echet Inception distance, coupled with a new technique that we propose to appraise the accuracy of virtual immunohistochemistry. This assesses the overlap between each stain component in the inferred and ground truth images through colour deconvolution, thresholding and the Sorensen-Dice coefficient. Our modified loss function resulted in a Dice coefficient for the virtual stain of 0.78 compared with the real AE1/AE3 slide. This was superior to the unaltered CycleGAN's score of 0.74. Additionally, our loss function improved the Fr\'echet Inception distance for the reconstruction to 74.54 from 76.47. We, therefore, describe an advance in virtual restaining that can extend to other immunostains and tumour types and deliver reproducible, fast and readily accessible immunohistochemistry worldwide.

==> introduction/abstract_old.tex <==
\begin{abstract}
    Immunohistochemistry (IHC) is a valuable diagnostic tool in cancer pathology. However, it is expensive, time-intensive, and requires specialist labs and equipment to perform it; consequently, not every facility has the resources to provide it. Haematoxylin and Eosin (H\&E) is a routine stain used in standard practice. It is low-cost, fast, and is applied with standard equipment. However, it has a disadvantage, as H\&E does not differentiate between tissue types. The high contrast provided by IHC overcomes this limitation. If deep learning could offer a virtualised tool to translate between H\&E and IHC stains with a high level of accuracy, it would save time, money and extend access to IHC. This paper presents a loss function optimised for training CycleGANs to translate H\&E to IHC pan-cytokeratin AE1AE3 virtually.
    
    We trained our network on consecutive sections stained with H\&E and pan-cytokeratin AE1AE3. We applied a modified version of the Vahadane stain normalisation method to tackle the expected variations in H\&E and AE1AE3 Pan-cytokeratin staining across datasets. We then carried out image registration and alignment at the whole slide scale. We repeated the alignment process at increasing resolutions until we achieved cell-level alignment. Using our paired slides, we generated datasets of varying patch sizes to train a CycleGAN to translate H\&E to AE1AE3. We prepared two networks; The first had the same loss functions used in the original CycleGAN. The second had a custom loss function that modifies the original loss function by removing identity loss and includes a term titled “mid-cycle” loss to compare the ground truth and generated patches in the middle of the training cycle. This modified loss function encourages accurate staining and authentic structural reproduction of the tissue. We used both networks to infer AE1AE3 stains on separate test slides, unseen to the network. We also present a new evaluation metric for virtual immunohistochemistry; the staining dice coefficient (SDC). We found that adding a mid-cycle loss component resulted in an SDC of 0.78 for the inferred AE1AE3 stain, compared to 0.74 for the original function. It also increased the SDC of the Haematoxylin stain to 0.86 vs the unaltered CycleGANs SDC score of 0.71. Additionally, mid-cycle loss also improved the Fr\'echet Inception Distance to 74.54 vs 76.47 for the original. Our success in inferring a specific IHC marker from the routine H\&E stain demonstrates the benefit of a deep learning technique for virtual IHC staining. We hope this method could be extended to other stains and tissue types and deliver cheaper, faster and readily accessible IHC staining.
\end{abstract}

%----------
% Narrative
%----------

% Confirm virtual immunohistochemistry (vIHC) from H\&E is possible with high structural reproduction and stain accuracy for resected colorectal cancer sections using A.I, trained with serial sections.

% Introduce novel loss function for improved stain accuracy based on comparing real and inferred patches at the midpoint of the CyleGANs training step from matched serial sections with similar tissue structure.

% Demonstrate its advantages over standard GAN/CycleGAN and its ability to work with “semi-paired” serial sections.

% Argue benefits of vIHC for use in speeding diagnosis + improving accuracy, reducing costs and positively impacting cancer outcomes.


==> methods/image_registration.tex <==
% \subsubsection{Whole Slide Registration and Realignment}

% Another requirement for our training dataset was that our paired serial sections were aligned down to the cellular level. This would allow us to train a deep network to convert the staining of structures across paired slides. We carried out whole-slide registration and realignment to address the structural divergence between serial sections. This is the process of finding similar features between a fixed and target slide and calculating an image transform to realign the target slide to the fixed slide.

% The first hurdle we faced in the image registration process was the visual disparity of H\&E and AE1AE3 slides. We tried several intensity-based image similarity metrics, none of them proved viable. Therefore, we attempted a mutual information metric; Specifically, the Mattes mutual information method \cite{mattes_nonrigid_2001}. Mutual information metrics measure how related two images are. They use the joint probability distribution of a sample of pixels at corresponding locations in both images to measure the confidence that the values from the fixed image map to similar values in the moving image \cite{mattes_pet-ct_2003}. A high mutual information score implies a reduction in the entropy between the two distributions. Therefore a higher mutual information score means that the images are better aligned and provides the algorithm with a parameter to optimise.

% Our image registration and realignment process is partitioned into stages to accommodate the gigapixel size of whole slide images within our available RAM. The first step was performing a rigid realignment with rotation, translation and isotropic scaling. However, because of the large dimensionality of the 20x whole slide images, we could not hold both in RAM to perform the registration process when they were at full resolution and uncompressed. To get around this, we performed the registration at half resolution and then scaled the parameters of the resulting transform to apply it to the full resolution image.

% We performed two additional registration and resampling rounds once the fixed and moving WSIs were approximately aligned using a rigid alignment. In the first of these, we tiled the WSI image into patches of size 11,000$^2$. We filtered out any patches where white pixels made up more than 95\% of the patch. Next, an affine transform was applied involving translation, rotation, isotropic scaling and sheer. Finally, the affine transform was combined with a deformable displacement field transform. A displacement field transform uses points placed in a grid over the images that relate to the image features underneath. Each point's required magnitude and displacement direction are calculated and represented as a vector. The desired result is to bring each point on the moving image into perfect alignment with its partner point and image feature in the fixed image. This transform calculates the deformation of the tissue in the serial section necessary to have the tissue structure match on a cellular level.
% In the last step, this affine-displacement field transform combination was repeated at the finest scale as the results from the previous step were tiled into patches of size 5000$^2$. This aligned the tissue with the accuracy necessary to train a deep network to convert stains. Finally, we split the tiles into a variety of patch sizes, determined by the input requirements of the network that we were to train.
